Lalaine: Measuring and Characterizing Non-Compliance of Apple Privacy Labels at Scale

As a key supplement to privacy policies that are known to be lengthy and difficult to read, Apple has launched the app privacy labels, which purportedly help users more easily understand an app's privacy practices. However, false and misleading privacy labels can dupe privacy-conscious consumers into downloading data-intensive apps, ultimately eroding the credibility and integrity of the labels. Although Apple releases requirements and guidelines for app developers to create privacy labels, little is known about whether and to what extent the privacy labels in the wild are correct and compliant, reflecting the actual data practices of iOS apps. This paper presents the first systematic study, based on our new methodology named Lalaine, to evaluate data-flow to privacy-label (flow-to-label) consistency. Lalaine analyzed the privacy labels and binaries of 5,102 iOS apps, shedding light on the prevalence and seriousness of privacy-label non-compliance. We provide detailed case studies and analyze root causes for privacy label non-compliance that complements prior understandings. This has led to new insights for improving privacy-label design and compliance requirements, so app developers, platform stakeholders, and policy-makers can better achieve their privacy and accountability goals. Lalaine is thoroughly evaluated for its high effectiveness and efficiency. We are responsibly reporting the results to stakeholders.

==> authors.tex <==

\author{\IEEEauthorblockN{1\textsuperscript{st} Given Name Surname}
\IEEEauthorblockA{\textit{dept. name of organization (of Aff.)} \\
\textit{name of organization (of Aff.)}\\
City, Country \\
email address or ORCID}
\and
\IEEEauthorblockN{2\textsuperscript{nd} Given Name Surname}
\IEEEauthorblockA{\textit{dept. name of organization (of Aff.)} \\
\textit{name of organization (of Aff.)}\\
City, Country \\
email address or ORCID}
\and
\IEEEauthorblockN{3\textsuperscript{rd} Given Name Surname}
\IEEEauthorblockA{\textit{dept. name of organization (of Aff.)} \\
\textit{name of organization (of Aff.)}\\
City, Country \\
email address or ORCID}
\and
\IEEEauthorblockN{4\textsuperscript{th} Given Name Surname}
\IEEEauthorblockA{\textit{dept. name of organization (of Aff.)} \\
\textit{name of organization (of Aff.)}\\
City, Country \\
email address or ORCID}
\and
\IEEEauthorblockN{5\textsuperscript{th} Given Name Surname}
\IEEEauthorblockA{\textit{dept. name of organization (of Aff.)} \\
\textit{name of organization (of Aff.)}\\
City, Country \\
email address or ORCID}
\and
\IEEEauthorblockN{6\textsuperscript{th} Given Name Surname}
\IEEEauthorblockA{\textit{dept. name of organization (of Aff.)} \\
\textit{name of organization (of Aff.)}\\
City, Country \\
email address or ORCID}
}


==> main/3.0.formulation.tex <==
\section{Problem Formulation}
motivation: why aggregate different purposes for the same data?

a certain inconsistency occurs simultaneously between label-code and label-policy -- indicates the process to generate label from policy is problematic, while the policy correctly reflects code behaviour; -- the label cannot correctly reflect privacy-sensitive code behavior

property of inconsistency (transitivity)
a certain inconsistency occurs between label-code while not in label-policy -- indicates the same inconsistency occurs between policy-code -- indicates the process to summarize policy from data behaviour is problematic, while the label correctly reflects the policy; -- the label cannot correctly reflect privacy-sensitive code behavior

a certain inconsistency occurs between label-policy while not in label-code -- indicates the same inconsistency occurs between policy-code -- indicates both processes to summarize policy from data behaviour and to summarize label from policy are problematic; However, the label can correctly reflect  privacy-sensitive code behavior;

\vspace{2pt}\noindent\textbf{Privacy label modeling.} 
We denoted $D_{t}$ to be 32 data objects (e.g., \textit{Email Address, Phone Number etc.}) defined by Apple that should be disclosed in privacy label if collected. Let $P_{t}$ represent the 6 purposes (e.g., \textit{Third-Party Advertising, Analytics, etc.}) also defined by Apple. We model an app’s privacy label as a set of tuple $R(D_{t}, P_{t}) = \{r|r:(d_{r},p_{r}), d_{r} \in D_{t}, p_{r} \subset P_{t})\}$. Each tuple $r$ represent a piece of data collection practice which clearly describe which data ($d_{r}$) is used for what purposes ($p_{r}$). Note that $p_{r}=\{p_{i}|p_{i}\in P_{t}\}$ can be a set of purposes as a data object can be used for multiple purposes. For example, ``Device ID" can be used for both \textit{Analytics} and \textit{Third-Party Advertising} purposes. 

\vspace{2pt}\noindent\textbf{Purpose Portfolio.} 

\ignore{
\subsection{Problem formalization}
As required by Apple, the developer need to correctly disclose what data is collected and how it is used from app’s privacy practices by comparing it with 32 data types and 6 purposes pre-defined by Apple \cite{}. Given an app, we can directly expand each data and its corresponding purpose from structural privacy label. For privacy policy, however, we need to extract sensitive data objects and identify its purposes from a set of the privacy policy statements \cite{policyLint}.

\vspace{2pt}\noindent\textbf{Privacy label modeling.} 
We denoted $D_{t}$ to be 32 data objects (e.g., \textit{Email Address, Phone Number etc.}) defined by Apple that should be disclosed in privacy label if collected. Let $P_{t}$ represent the 6 purposes (e.g., \textit{Third-Party Advertising, Analytics, etc.}) also defined by Apple. We model an app’s privacy label as a set of tuple $R(D_{t}, P_{t}) = \{r|r:(d_{r},p_{r}), d_{r} \in D_{t}, p_{r} \subset P_{t})\}$. Each tuple $r$ represent a piece of data collection practice which clearly decribe which data ($d_{r}$) is used for what purposes ($p_{r}$). Note that $p_{r}=\{p_{i}|p_{i}\in P_{t}\}$ can be a set of purposes as a data object can be used for multiple purposes. For example, ``Device ID" can be used for both \textit{Analytics} and \textit{Third-Party Advertising} purposes. 


\vspace{2pt}\noindent\textbf{Privacy policy modeling.} We model an app’s privacy policy as a set of tuple $S(D_{s}, P_{t}) = \{s|s:(d_{s},p_{s}), d_{s} \in D_{s}, p_{s} \subset P_{t})\}$. Here $D_{s}$ represents the total set of data objects extracted by PolicyLint, $P_{t}$ has been defined above (6 purposes defined by Apple), $p_{s}=\{p_{s}|p_{s}\in P_{t}\}$ are a set of purposes after alignment using table~\ref{table:purpose_alignment}.


}




\subsection{Inconsistency Model between \LX{Privacy Label and Privacy Policy}}

\vspace{2pt}\noindent\textbf{Inconsistent type.} Ideally, for each data collection and purpose $s=(d_{s},p_{s})$ in privacy policy, if $d_{s}$ can be aligned with any data type $d_{r}$ in $D_{t}$, then $(d_{r},p_{s})$ should be disclosed in privacy label. This is a consistent disclosure between privacy policy and privacy label based on Apple's policy \textit{``The developer need to provide information about your app’s privacy practices''}.
%The purpose of the label is to help your customers understand what data is collected from your app and how it is used.

%   
Inconsistency can occur at both data level and purpose level. Here, we defined three inconsistency types. They are \textit{Omitted Disclosure}, \textit{Incorrect Disclosure}, and \textit{Inadequate Disclosure} respectively. 
%
%Given an app's privacy policy, we first extract a set of $S$ where $s = (d_{s},p_{s})$, $s \in S$. Given an app's privacy label, we extract a set of $R$ where $r = (d_{r},p_{r})$, $r \in R$.


\ignore{
\vspace{2pt}\noindent\textbf{Definition.}

$d_{s}\equiv_{o}d_{r}$ or $d_{s}\sqsubset_{o}d_{r}$ or $d_{s}\sqsupset{o}d_{r}$

\begin{itemize}
  \item \textbf{Omitted Disclosure}. 
  Given $s = (d_{s},p_{s})$, $\forall r = (d_{r},p_{r}), r \in R$, s.t.  there is no $d_{s}\equiv_{o}d_{r}$ or $d_{s}\sqsubset_{o}d_{r}$ or $d_{s}\sqsupset{o}d_{r}$, then $s = (d_{s},p_{s})$ is considered as an omitted disclosure for privacy label. 
 \qy{then xxx r is s omitted disclosure}
 
 

  \item \textbf{Incorrect Disclosure}.  Given $s = (d_{s},p_{s})$, if there exists $r = (d_{r},p_{r})$, which makes $d_{s}\equiv_{o}d_{r}$ or $d_{s}\sqsubset_{o}d_{r}$ or $d_{s}\sqsupset_{o}d_{r}$, but $p_{s}\neq p_{r}$.
  
    \item \textbf{Inadequate Disclosure}. Given $s = (d_{s},p_{s})$, if there exists $r = (d_{r},p_{r})$, which makes $d_{s}\equiv_{o}d_{r}$ or $d_{s}\sqsubset_{o}d_{r}$ or $d_{s}\sqsupset{o}d_{r}$, but $p_{r}\sqsubset p_{s}$.
  
\end{itemize}
}

------------------


Given a privacy policy statement $s = (d_{s},p_{s})$, we define its \textit{associated privacy label} as
$\mathcal{R}(s) = \{r:(d_r,p_r)|d_r: d_{s}\equiv_{o}d_{r} \vee d_{s}\sqsubset_{o}d_{r} \vee d_{s}\sqsupset_{o}d_{r}\}$, where the data object in the associated privacy label is either a synonym, a hypernym, or a hyponym of the data object  in the privacy policy statement. 
%
Let $\mathcal{P}_{\mathcal{R}(s)} = \{p_r|(d_r,p_r)\in \mathcal{R}(s)\}$ denote the purposes in the associated privacy label of statement $s$.
%
According to the results of the atomic alignment on the data objects and the purposes, we define three inconsistency relationship between a privacy policy statement $s$ and the privacy label $R$ as below. 

\begin{inconsistency}[${[\nVDash]}$ Omitted Disclosure] The privacy label $R$ is an \textit{omitted disclosure} with regard to a privacy policy statement $s$ if there exists no associated privacy label for the statement: 
\[
\mathcal{R}(s) = \emptyset \ \Rightarrow \ R \nVDash s
\]
\end{inconsistency} 
\begin{inconsistency}[${[\nvDash]}$ Incorrect Disclosure] 
The privacy label $R$ is an \textit{incorrect disclosure} with regard to a privacy policy statement $s$ if the associated privacy label $\mathcal{R}(s)$ exists while the purposes in $\mathcal{R}(s)$ \textit{disaccord} with those in the statement:
\[
\mathcal{R}(s)\neq \emptyset \ \wedge\ \exists p \in \mathcal{P}_{\mathcal{R}(s)}, p \notin p_s   \wedge  p_s \nsubseteq \mathcal{P}_{\mathcal{R}(s)} \  \ \Rightarrow \ R \nvDash s
\]
\end{inconsistency}

\begin{inconsistency}[${[\nvdash]}$ Inadequate Disclosure] 
The privacy label $R$ is an \textit{inadequate disclosure} with regard to a privacy policy statement $s$ if the associated privacy label $\mathcal{R}(s)$ exists while the purposes in $\mathcal{R}(s)$ is a \textit{proper subset} of those in the statement:
\[
\mathcal{R}(s)\neq \emptyset \ \wedge\ \mathcal{P}_{\mathcal{R}(s)} \subset p_s \  \ \Rightarrow \ R \nvdash s
\]

\end{inconsistency}

\ignore{
close the research gap: inconsistency with the same sentiment. 

% \section{Problem Formulation}
motivation: why aggregate different purposes for the same data?

a certain inconsistency occurs simultaneously between label-code and label-policy -- indicates the process to generate label from policy is problematic, while the policy correctly reflects code behaviour; -- the label cannot correctly reflect privacy-sensitive code behavior

property of inconsistency (transitivity)
a certain inconsistency occurs between label-code while not in label-policy -- indicates the same inconsistency occurs between policy-code -- indicates the process to summarize policy from data behaviour is problematic, while the label correctly reflects the policy; -- the label cannot correctly reflect privacy-sensitive code behavior

a certain inconsistency occurs between label-policy while not in label-code -- indicates the same inconsistency occurs between policy-code -- indicates both processes to summarize policy from data behaviour and to summarize label from policy are problematic; However, the label can correctly reflect  privacy-sensitive code behavior;

\vspace{2pt}\noindent\textbf{Privacy label modeling.} 
We denoted $D_{t}$ to be 32 data objects (e.g., \textit{Email Address, Phone Number etc.}) defined by Apple that should be disclosed in privacy label if collected. Let $P_{t}$ represent the 6 purposes (e.g., \textit{Third-Party Advertising, Analytics, etc.}) also defined by Apple. We model an app’s privacy label as a set of tuple $R(D_{t}, P_{t}) = \{r|r:(d_{r},p_{r}), d_{r} \in D_{t}, p_{r} \subset P_{t})\}$. Each tuple $r$ represent a piece of data collection practice which clearly describe which data ($d_{r}$) is used for what purposes ($p_{r}$). Note that $p_{r}=\{p_{i}|p_{i}\in P_{t}\}$ can be a set of purposes as a data object can be used for multiple purposes. For example, ``Device ID" can be used for both \textit{Analytics} and \textit{Third-Party Advertising} purposes. 

\vspace{2pt}\noindent\textbf{Purpose Portfolio.} 

\ignore{
\subsection{Problem formalization}
As required by Apple, the developer need to correctly disclose what data is collected and how it is used from app’s privacy practices by comparing it with 32 data types and 6 purposes pre-defined by Apple \cite{}. Given an app, we can directly expand each data and its corresponding purpose from structural privacy label. For privacy policy, however, we need to extract sensitive data objects and identify its purposes from a set of the privacy policy statements \cite{policyLint}.

\vspace{2pt}\noindent\textbf{Privacy label modeling.} 
We denoted $D_{t}$ to be 32 data objects (e.g., \textit{Email Address, Phone Number etc.}) defined by Apple that should be disclosed in privacy label if collected. Let $P_{t}$ represent the 6 purposes (e.g., \textit{Third-Party Advertising, Analytics, etc.}) also defined by Apple. We model an app’s privacy label as a set of tuple $R(D_{t}, P_{t}) = \{r|r:(d_{r},p_{r}), d_{r} \in D_{t}, p_{r} \subset P_{t})\}$. Each tuple $r$ represent a piece of data collection practice which clearly decribe which data ($d_{r}$) is used for what purposes ($p_{r}$). Note that $p_{r}=\{p_{i}|p_{i}\in P_{t}\}$ can be a set of purposes as a data object can be used for multiple purposes. For example, ``Device ID" can be used for both \textit{Analytics} and \textit{Third-Party Advertising} purposes. 


\vspace{2pt}\noindent\textbf{Privacy policy modeling.} We model an app’s privacy policy as a set of tuple $S(D_{s}, P_{t}) = \{s|s:(d_{s},p_{s}), d_{s} \in D_{s}, p_{s} \subset P_{t})\}$. Here $D_{s}$ represents the total set of data objects extracted by PolicyLint, $P_{t}$ has been defined above (6 purposes defined by Apple), $p_{s}=\{p_{s}|p_{s}\in P_{t}\}$ are a set of purposes after alignment using table~\ref{table:purpose_alignment}.


}
}

\ignore{
\vspace{2pt}\noindent\textbf{Definition.}

$d_{s}\equiv_{o}d_{r}$ or $d_{s}\sqsubset_{o}d_{r}$ or $d_{s}\sqsupset{o}d_{r}$

\begin{itemize}
  \item \textbf{Omitted Disclosure}. 
  Given $s = (d_{s},p_{s})$, $\forall r = (d_{r},p_{r}), r \in R$, s.t.  there is no $d_{s}\equiv_{o}d_{r}$ or $d_{s}\sqsubset_{o}d_{r}$ or $d_{s}\sqsupset{o}d_{r}$, then $s = (d_{s},p_{s})$ is considered as an omitted disclosure for privacy label. 
 \qy{then xxx r is s omitted disclosure}
 
 

  \item \textbf{Incorrect Disclosure}.  Given $s = (d_{s},p_{s})$, if there exists $r = (d_{r},p_{r})$, which makes $d_{s}\equiv_{o}d_{r}$ or $d_{s}\sqsubset_{o}d_{r}$ or $d_{s}\sqsupset_{o}d_{r}$, but $p_{s}\neq p_{r}$.
  
    \item \textbf{Inadequate Disclosure}. Given $s = (d_{s},p_{s})$, if there exists $r = (d_{r},p_{r})$, which makes $d_{s}\equiv_{o}d_{r}$ or $d_{s}\sqsubset_{o}d_{r}$ or $d_{s}\sqsupset{o}d_{r}$, but $p_{r}\sqsubset p_{s}$.
  
\end{itemize}
}


==> main/4.overview_of_privacy_label.tex <==
\section{Ecosystem Overview: a Longitudinal Analysis}

In this section, we present an overview of the ecosystem of privacy label. In particular, our study reveals an increasing trend of app with privacy labels. 

\subsection{Pervasiveness of privacy label}

\ignore{
\subsubsection{How many app has privacy label, longitudinal change from no provide details to collect data, Lifespan of privacy label}
}
%




\vspace{2pt}\noindent\textbf{Scope and magnitude}. 
%
From our seven-month longitudinal dataset between Nov, 2021 and May, 2022, given 485,024 APP bundle IDs, we gathered 204,924 unique apps (42.3\%) that employed privacy label to declare data collection and usage information. 
%
Figure~\ref{fig:numPrivacyLabl} shows the number of unique iOS apps and their associated privacy labels per week. The weeks without bars in the plot are missing data due to the functionality issues of our data crawler.


On average, we collected 20 snapshots and 20 \xiaojing{????} unique privacy labels for each iOS app. 
%
%The sudden increase of the number of apps with privacy label since Jan 24, 2022 was due to the additional bundle IDs in our dataset. 
From the figure, we observed that the number of apps with privacy label is generally stable during our crawling period.
%
In our study, we found that 12,721 apps in total updated their privacy labels from ``Not provide details'' to any one of other four data categories during our observation period. The figure shows that the number of apps made such change between our two crawling slot is between 336 and 1,590. Even though the number of newly appeared privacy labels is comparatively small, it indicates a gradually increasing trend of the apps with privacy label.
%
\zhengyi{The red line in Figure~\ref{fig:numPrivacyLabl} shows the number of ``disappeared'' apps for each crawling round in our dataset. Those apps might be deleted from Apple Store forever, or our crawler failed in collecting them in that snapshot period.}
%\xiaojing{add disappear trend; discuss the cases of newly-appear and disappeared}
%\xiaojing{the figure and number look inconsistent; need discuss here}

\begin{figure}[t]
    \centering
    \includegraphics[width=\columnwidth]{figure/dateNumPrivacyLabel.pdf}
    \caption{The number of unique iOS apps and their associate privacy labels per week. The blue area at the bottom of each bar shows the number of unique iOS apps with newly appeared privacy labels (i.e., privacy label changes from ``Not provide details'' to any other data category).}
    \label{fig:numPrivacyLabl}
\end{figure}


Apps with privacy labels, as collected in our dataset, are found in all 26 categories of the Apple App Store (except Safari Extensions category). The top five categories are: Games (14.3\%), Education (8.5\%), Business (8.3\%), Lifestyle (7.3\%), and Utilities (6.8\%).
%
We also studied the rating of those apps with privacy label. We observed that most apps (58\%) have a rating between 3.0 - 5.0.
%
%We found that xx (xx\%) apps are of high ranks. XX apps were in the top 100 of their corresponding category.




\vspace{2pt}\noindent\textbf{Categories of privacy labels}. 
%
To study the categories of privacy labels covered in this study, we look into 23 snapshots of 8,143,213 privacy labels from Nov, 2021 to May, 2022. 
%
We notice that among four categories of data usage in high level, ``Data Not Linked to You'' is the most which is claimed by 91,720 (34\%) apps, followed by ``Data Linked to You'' claimed by 73,331 (27.3\%) apps, ``Data Not Collected'' (20.8\%) and ``Data Used to Track You'' (18\%). We observe that those four categories remain stable in the reported data collection, which generally aligns with the findings in~\cite{privacyNutrition}. However, we do not find a decrease trend in ``Data Used to Track You''. It might because the decreasing trend starting from late April, 2021 reaches to a stable condition as the time we started to collect privacy label data.
%
%\xiaojing{discuss the general trend}

\input{table/privacyLabelBreakdown}


Looking into the privacy labels of ``Data Linked to you'' and ``Data used to Track you'', Table~\ref{table:labelBreakdown} shows the breakdown of privacy label into each data type/data usage over the seven-month span (Nov, 2021 and May, 2022).
%
We observe that the most popular purpose of data usage is App Functionality (33.4\%), followed by Analytics (23.3\%) and Product Personalization (15.7\%). According to the definition of data use in ~\cite{iosprivacylabel}, all those three purposes are highly related to individual user's behavior and/or customization. For instance, App Functionality purpose includes apps' activities like users authentication, customer support, implement of security measures, etc.
%
Meanwhile, the top-3 data types are Identifiers, Usage Data, and Contact Info, while the most type of data item being collected is Device ID, followed by User ID and Email Address.
%
Particularly, Device ID and User ID are the only two data items within Identifiers data type and the most popular data items, indicating most apps incline to use the existing system generated and easy-to-collected ID as identifier to track or link the app to specific users, rather than using names or email address, which require users to type in submission form before collection.
%
%It is clear that the most popular data types align with the top purposes of the data usage. 
%\xiaojing{this part should be discussed}

\begin{figure}[t]
    \centering
    \includegraphics[width=\columnwidth]{figure/newly_appeared.pdf}
    \caption{Number of newly-appeared popular purpose and data items within ``Data Linked to you'' and ``Data used to Track you'' categories.}
    \label{fig:newlyAppearedLabel}
\end{figure}

\begin{figure}[t]
    \centering
    \includegraphics[width=\columnwidth]{figure/disppeared.pdf}
    \caption{Number of disappeared popular purpose and data items within ``Data Linked to you'' and ``Data used to Track you'' categories.}
    \label{fig:disappearedLabel}
\end{figure}


\vspace{2pt}\noindent\textbf{Evolution of privacy label.} 
%\xiaojing{add the figure of newly-apear/disappear data usage purposes (link to you/trace you)}
Privacy label is dynamic and evolved over time as the development and update of apps.
%
To study such phenomenon, we combine the dataset of 23 snapshots (7,583,958 privacy labels) and achieved 412,340 apps which appeared in at least two snapshots from Nov, 2021 to May, 2022. In total, we observed 27,060 changes happened on privacy labels. Among them, 18,175 (4.4\% of total apps) apps' privacy labels changed at least once.
%
In our study, within the categories of ``Data Linked to you'' and ``Data used to Track you'', we observe ``App Functionality'', ``Analytics'' and ``'Product Personalization'' are the top-3 newly-appeared purpose of data usage, while ``Identifiers'', ``Usage Data'' and ``Contact Info'' are the top-3 newly-added data types. The trend of those newly-appeared popular data purpose and data types over time is shown in Figure~\ref{fig:newlyAppearedLabel}. Notice that we consider an item in privacy label as newly-appeared if it was not claimed in the previous most recent crawling result.
%
We notice four peaks involving a large amount of newly-appeared purpose and data types happened on Nov 2021, Dec 2021, middle of Feb 2022, and April 2022. From Figure~\ref{fig:numPrivacyLabl}, however, we did not see a great change of newly-appeared privacy labels in above periods. We guess those mass newly-added purposes and data items are made due to app developers' regular updating by introducing new features to their iOS apps.
%
For example, \href{E.D.GymsHero}{E.D.GymsHero} said ``Meet the new analytics section! We've added analyses of your training so you can keep track of your progress...'' in its version history updated on Jan 3, 2022, after we noticed the new Analytics purpose appeared on its privacy label.
%

\ignore{It is highly possible that some new features are introduced to those apps, leading to the adjustment on data collection types and purpose of data usages.} 
%\xiaojing{find a more insteresting case here}
%\xiaojing{some case studies here}.
%

Meanwhile, we also study the disappeared purposes and data types in privacy label. Particularly, ``Analytics'', ``App Functionality'' and ``Third-Party Advertising'' are the top-3 newly-removed purpose of data usage, while ``Identifiers'', ``Usage Data'' and ``Location'' are the top-3 newly-deleted data types. Figure~\ref{fig:disappearedLabel} shows the trend over time.
%
We looked into those apps' version history and tried to find the reason for the removal. We observed that some of those apps terminated some functionalities or stopped collaboration with third parties, For instance, \href{com.artsolution.kidsdrawing}{com.artsolution.kidsdrawing} mentioned it ``Removed google analytics.'' on May 11, 2022, after we noticed the corresponding Analytics purpose was removed on May 2, 2022. 
%
We also hypothesize that privacy label makes data being collected by apps more transparent to end users. In this case, those apps begin to inspect themselves and try not to aggressively claim data collection information.
%
%We also found some apps stealthy removed the purpose/data types in privacy label without mentioning any changes in their version history. For instance, xxx.

%\xiaojing{some case studies here}.
%\xiaojing{did we conduct a dynamic analysis on them?}

%
Surprisingly, we observe 239 apps changed their privacy labels from collecting data (either \textit{Data Used to Track You}, \textit{Data Linked to You}, or \textit{Data Not Linked to You}) to either ``Data Not Collected'' (97\%) or ``Not Provide Details'' (3\%). 
%
Looking into those apps, we found that such abnormal change happened all the time during our crawling period. The data that those app used to collected covered all 3 categories of data usage, 6 purposes of data usage, 14 data types and 32 specific data items. 
%
For example, \href{com.mmi.mmievents}{com.mmi.mmievents}'s privacy label shown it collected 8 different data types and 17 specific data items before Feb 28, 2022, which is the most among all those apps. After that date, its privacy label become ``Data Not Collected'' till now (May 26, 2022). Its version history shows the most recent update was ``Updated App Icon and Screenshots'' on Mar 18, 2022, without mentioning anything about the change in data collection and usage information. It is unlikely that this app suddenly made huge changes on its functional operations, because it has been four years since its release and been updating all the time as early as 2018.
%

To understand why those apps just all of a sudden began to ``not collect data'', we conduct a dynamic analysis on XX of those apps, as elaborated on Section XX.



%the CDF of those apps by the number of them changing the privacy label status every week. Averagely, around 537 apps will update their privacy label weekly to provide their data collection information in privacy label. It implies the increasing trend of the popularity of privacy label. \xiaojing{to discuss}



%From the table, we find that xxx category collect xxx, which align with ~\cite{xxx}. It also generally implies that the privacy label are accurate at some level.


%
%Among them, 138,647 (68.3\%) apps have at least one category (either Data used to track you, Data Not Linked to You, or Data Linked to You) in privacy label, which imply they will collect data during the apps' usage. While 65,840 (32.4\%) apps declare that they do not collect any kind of data, with privacy label showing ``Data Not Collected''.

%
%For the remaining 222,887 (53.9\%) apps, they do not provide any information about data collection and usage. Their privacy label basically shows ``Not Provide Details''. It is possible that those apps haven't updated their privacy label in App Store in time, because we observed 11,266 (5.1\% among the remain) apps have changed the privacy label status from ``Not provide details'' to any one of other four  during our crawling period. 


%Altogether, privacy label, which serves as an useful tool to offer data collection details to end-users, is popular and pervasive in all app categories and within apps with different ranks and ratings.




\vspace{2pt}\noindent\textbf{Supplement other privacy disclosures}.
Here, we aim to investigate whether privacy label supplements the privacy disclosure.
%
More specifically, we investigate the apps with at least one privacy disclosure, either privacy label or privacy policy, is available for users to look for data being collected by the apps.
%
Here we consider privacy label to be unavailable if it is ``Not Provide Details''. The privacy policy is unavailable if the developer’s privacy policy link in the app download page does not return a valid response. Note that we did not consider in-app privacy disclosures in this study.
%
To this end, based on our most recent scraping result on May 9, 2022, among 340,095 iOS apps, we found 144,595 (42.5\%) of them with only privacy policies, 22,894 (6.7\%) with only privacy labels. Surprisingly, we also observed 14,753 (4.3\%) apps with neither privacy disclosures.
%
For instance, \href{com.fareness.fareness}{com.fareness.fareness} has 9.1K ratings and 4.6 rating score, while its privacy label is lacking and privacy policy returns 404 error, indicating the mass users have no idea about data collection and usage information. By performing dynamic analysis on this app, we found that it actually collected payment information and xxx.
 
%\xiaojing{some case studies here}

%\vspace{2pt}\noindent\textbf{Supplement other privacy disclosures}.
%\xiaojing{App without correct privacy policy, whether it provides privacy label}
%\xiaojing{App without privacy label (No details provided type), whether provide correct policy link (return code, return content [policyLint to collect policy statement sentence])}


%%% num of app make any changes to privacy label

\ignore{
\begin{figure}[t]
    \centering
    \includegraphics[width=\columnwidth]{figure/weeklyUpdate_noDetailsOthers.pdf}
    \caption{Weekly updated apps.}
    \label{fig:weeklyUpdate}
\end{figure}
}
%life span



\subsection{Latency Analysis}
%\vspace{2pt}\noindent\textbf{Duration between the updated of PL and PP}
%\xiaojing{Privacy policy update time VS Privacy label update time (latency analysis)}

%\vspace{2pt}\noindent\textbf{Duration between the updated of PL and Apps}
We study whether app developers respond to the request of Apple to include privacy label when publishing apps~\cite{} in a timely manner.
%
In particular, we investigate the time span between app's version update and the time when the first privacy label appearing.
%
To this end, among 12,721 apps whose privacy labels changed from ``Not Provide Details" to any others, we collected their version histories, which consist of all previous versions and their corresponding update time, in the app download pages. 
%
We first located the timestamp when the privacy label first appear, as well as the most recent date (toward that timestamp) when the version history update. We then calculated the latency in days between those two dates. %
Typically, to eliminate the influence of the delay of our scraping work, we excluded the latency days which are less than seven days to get a lower boundary of such latency.
%
In our study, we observed 6,109 (48\%) apps did not update in time, with an average latency of 59.5 days. Among them, we still haven't seen 3,323 (54.4\%) apps making any update till the last crawl (May 12, 2022).
%
For example, com.swiftappskom.thetigerrpg, a game app with 9K ratings, first shown its privacy label on April 11, 2022. Till now (Jun 6, 2022), however, we haven't seen any updates on its version history.

Surprisingly, when matching the privacy label updates and their associated app updates, we observe 1,088 (17.6\%) apps kept updating their privacy labels but with the apps never being updated. The remain 2,871 (46.3\%) apps did not update their version history in time with averagely 44.1 days latency.
%
As an instance, \href{com.creagames.clashoflegions}{com.creagames.clashoflegions} updated its privacy label by adding Third-Party Advertising purpose and adding Identifiers and Device ID data types on Dec 6, 2021. The version of this app did not updated until Dec 15, 2021, mentioned that it has ``added advertising function''.
%\xiaojing{Also discuss other suspicious scenarios}



%Specifically, we tracked privacy label change (either data types or data usage purpose change happened) weekly from our longitudinal dataset and used the start day of that week as the date when privacy label change are noticed. Next we followed the Version History and used the most recent version update date (after the privacy label change date) to calculate the latency between it and the privacy label change date. If the version of app has never been updated, we consider the latency to be infinite. For example, suppose we notice that the privacy label changed on April 17, 2022, the version is updated on May 9, 2022, the latency is 23 days.

%Table~\ref{table:xxx} illustrates the latency. From the table, we notice that xxx

%\xiaojing{The time gap between the update of privacy label and version (latency analysis: eg.,  latest privacy label update at 5/07/2022, but software version latest update at 4/07/2022,  there is one month duration of missing correct privacy label)}

%\zhengyi{for those not privde details, do they update what's new? does updating what's new sychro with updating privacy label?}

\subsection{Uniqueness of Privacy Label}
In our study, we found that privacy label provides a better app-specific privacy disclosure, compared with privacy policy.
%
Particularly, among 29,034 groups of privacy policies which are shared by 138,493 apps (on average 5 apps per privacy policies), we observe the average percent of unique privacy labels is 82.1\%. 8592 (29.6\%) of groups have at least one different privacy labels for the apps in the group. 
%
We hypothesize that those apps might be developed by the same developer or app generator, causing them use the same privacy policy. For example, Subsplash Platform~\cite{Subsplash} provide services to build church mobile app and websites and have its privacy policy being shared by 1,856 apps. However, their privacy labels were specifically created based on the app's actual data collections and usage, causing them have app-specific privacy label.
%
As an instance, 16 unique privacy labels are observed for the aforementioned Subsplash privacy policy~\cite{Subsplash}. The data collection and usage of purposes are completely different. One of the privacy label even claimed it does not collect any data.
%
%
This indicates that it is hard to verify the correctness of privacy label only by analyzing the privacy policy, while it is supposed to extend privacy label with detailed data collection information for each app.
%

%To understand whether privacy label is specific for each app while privacy policy can be general for a group of apps, we focus on the apps whose have same developer's privacy policy link in Apple App Store.

%
%In total, we found xxx privacy policy are shared by xxx different apps. For example, xxxx is listed as privacy policy url for xxx unique apps. Among them, xx apps have different privacy policy label. %

%


%\xiaojing{Whether privacy policy is general, while privacy label is specific for one app (Analysis of same privacy policy link but different app privacy label)}
%\xiaojing{same privacy policy, different apps}
%\xiaojing{same privacy policy, privacy label difference in different apps}
%\xiaojing{same privacy policy, whether privacy label difference claimed in privacy policy}





==> main/5.comparison_between_privacy_label_and_privacy_policy.tex <==
\section{Inconsistency analysis between privacy label and privacy policy}
As mentioned earlier, privacy label lists the types and purpose of data being collected in an easily digestible format and is a concise representation of the privacy policy. 
%
To automatically check whether privacy label and privacy policy are consistent, we first collected privacy policy data and retrieved the target object (i.e., data items, data usage purpose, etc.). Then we mapped the target object to those used in privacy label to make the comparison possible. Finally we analyzed the pervasiveness, reason, and trend for the existence of inconsistency. 



\vspace{2pt}\noindent\textbf{Privacy policy modeling.} We model an app’s privacy policy as a set of tuple $S(D_{s}, P_{t}) = \{s|s:(d_{s},p_{s}), d_{s} \in D_{s}, p_{s} \subset P_{t})\}$. Here $D_{s}$ represents the total set of data objects, $p_{s}=\{p_{s}|p_{s}\in P_{t}\}$ represented as a set of purposes after alignment using table~\ref{table:purpose_alignment}. $P_{t}$ are the set of 6 purposes defined by Apple. \XY{need rewrite refer to section3}



\ignore{
\subsection{Problem formalization}
As required by Apple, the developer need to correctly disclose what data is collected and how it is used from app’s privacy practices by comparing it with 32 data types and 6 purposes pre-defined by Apple \cite{}. Given an app, we can directly expand each data and its corresponding purpose from structural privacy label. For privacy policy, however, we need to extract sensitive data objects and identify its purposes from a set of the privacy policy statements \cite{policyLint}.

\vspace{2pt}\noindent\textbf{Privacy label modeling.} 
We denoted $D_{t}$ to be 32 data objects (e.g., \textit{Email Address, Phone Number etc.}) defined by Apple that should be disclosed in privacy label if collected. Let $P_{t}$ represent the 6 purposes (e.g., \textit{Third-Party Advertising, Analytics, etc.}) also defined by Apple. We model an app’s privacy label as a set of tuple $R(D_{t}, P_{t}) = \{r|r:(d_{r},p_{r}), d_{r} \in D_{t}, p_{r} \subset P_{t})\}$. Each tuple $r$ represent a piece of data collection practice which clearly decribe which data ($d_{r}$) is used for what purposes ($p_{r}$). Note that $p_{r}=\{p_{i}|p_{i}\in P_{t}\}$ can be a set of purposes as a data object can be used for multiple purposes. For example, ``Device ID" can be used for both \textit{Analytics} and \textit{Third-Party Advertising} purposes. 


\vspace{2pt}\noindent\textbf{Privacy policy modeling.} We model an app’s privacy policy as a set of tuple $S(D_{s}, P_{t}) = \{s|s:(d_{s},p_{s}), d_{s} \in D_{s}, p_{s} \subset P_{t})\}$. Here $D_{s}$ represents the total set of data objects extracted by PolicyLint, $P_{t}$ has been defined above (6 purposes defined by Apple), $p_{s}=\{p_{s}|p_{s}\in P_{t}\}$ are a set of purposes after alignment using table~\ref{table:purpose_alignment}.







\subsection{Inconsistency model between PL and PP}

\vspace{2pt}\noindent\textbf{Inconsistent type.} Ideally, for each data collection and purpose $s=(d_{s},p_{s})$ in privacy policy, if $d_{s}$ can be aligned with any data type $d_{r}$ in $D_{t}$, then $(d_{r},p_{s})$ should be disclosed in privacy label. This is a consistent disclosure between privacy policy and privacy label based on Apple's policy \textit{``The developer need to provide information about your app’s privacy practices''}.
%The purpose of the label is to help your customers understand what data is collected from your app and how it is used.

%   
Inconsistency can occur at both data level and purpose level. Here, we defined three inconsistency types. They are \textit{Omitted Disclosure}, \textit{Incorrect Disclosure}, and \textit{Inadequate Disclosure} respectively. 
%
%Given an app's privacy policy, we first extract a set of $S$ where $s = (d_{s},p_{s})$, $s \in S$. Given an app's privacy label, we extract a set of $R$ where $r = (d_{r},p_{r})$, $r \in R$.


\ignore{
\vspace{2pt}\noindent\textbf{Definition.}

$d_{s}\equiv_{o}d_{r}$ or $d_{s}\sqsubset_{o}d_{r}$ or $d_{s}\sqsupset{o}d_{r}$

\begin{itemize}
  \item \textbf{Omitted Disclosure}. 
  Given $s = (d_{s},p_{s})$, $\forall r = (d_{r},p_{r}), r \in R$, s.t.  there is no $d_{s}\equiv_{o}d_{r}$ or $d_{s}\sqsubset_{o}d_{r}$ or $d_{s}\sqsupset{o}d_{r}$, then $s = (d_{s},p_{s})$ is considered as an omitted disclosure for privacy label. 
 \qy{then xxx r is s omitted disclosure}
 
 

  \item \textbf{Incorrect Disclosure}.  Given $s = (d_{s},p_{s})$, if there exists $r = (d_{r},p_{r})$, which makes $d_{s}\equiv_{o}d_{r}$ or $d_{s}\sqsubset_{o}d_{r}$ or $d_{s}\sqsupset_{o}d_{r}$, but $p_{s}\neq p_{r}$.
  
    \item \textbf{Inadequate Disclosure}. Given $s = (d_{s},p_{s})$, if there exists $r = (d_{r},p_{r})$, which makes $d_{s}\equiv_{o}d_{r}$ or $d_{s}\sqsubset_{o}d_{r}$ or $d_{s}\sqsupset{o}d_{r}$, but $p_{r}\sqsubset p_{s}$.
  
\end{itemize}
}

------------------


Given a privacy policy statement $s = (d_{s},p_{s})$, we define its \textit{associated privacy label} as
$\mathcal{R}(s) = \{r:(d_r,p_r)|d_r: d_{s}\equiv_{o}d_{r} \vee d_{s}\sqsubset_{o}d_{r} \vee d_{s}\sqsupset_{o}d_{r}\}$, where the data object in the associated privacy label is either a synonym, a hypernym, or a hyponym of the data object  in the privacy policy statement. 
%
Let $\mathcal{P}_{\mathcal{R}(s)} = \{p_r|(d_r,p_r)\in \mathcal{R}(s)\}$ denote the purposes in the associated privacy label of statement $s$.
%
According to the results of the atomic alignment on the data objects and the purposes, we define three inconsistency relationship between a privacy policy statement $s$ and the privacy label $R$ as below. 

\begin{inconsistency}[${[\nVDash]}$ Omitted Disclosure] The privacy label $R$ is an \textit{omitted disclosure} with regard to a privacy policy statement $s$ if there exists no associated privacy label for the statement: 
\[
\mathcal{R}(s) = \emptyset \ \Rightarrow \ R \nVDash s
\]
\end{inconsistency} 
\begin{inconsistency}[${[\nvDash]}$ Incorrect Disclosure] 
The privacy label $R$ is an \textit{incorrect disclosure} with regard to a privacy policy statement $s$ if the associated privacy label $\mathcal{R}(s)$ exists while the purposes in $\mathcal{R}(s)$ \textit{disaccord} with those in the statement:
\[
\mathcal{R}(s)\neq \emptyset \ \wedge\ \exists p \in \mathcal{P}_{\mathcal{R}(s)}, p \notin p_s   \wedge  p_s \nsubseteq \mathcal{P}_{\mathcal{R}(s)} \  \ \Rightarrow \ R \nvDash s
\]
\end{inconsistency}

\begin{inconsistency}[${[\nvdash]}$ Inadequate Disclosure] 
The privacy label $R$ is an \textit{inadequate disclosure} with regard to a privacy policy statement $s$ if the associated privacy label $\mathcal{R}(s)$ exists while the purposes in $\mathcal{R}(s)$ is a \textit{proper subset} of those in the statement:
\[
\mathcal{R}(s)\neq \emptyset \ \wedge\ \mathcal{P}_{\mathcal{R}(s)} \subset p_s \  \ \Rightarrow \ R \nvdash s
\]

\end{inconsistency}


% data collection practices in your app

}


\begin{figure}[t!]
\center
\includegraphics[width = 0.55 \textwidth]{figure/OmitDisclosurePP_PL.png}
\caption{Omitted Disclosure}
\label{fig:omit}
\end{figure}



\subsection{Pervasiveness of Inconsistency}
To understand the gap between privacy policy and privacy label,  we perform the measurement study on three types of inconsistency \textit{Omitted Disclosure}, \textit{Incorrect Disclosure}, and \textit{Inadequate Disclosure}.

\subsubsection{Omitted Disclosure}
Omitted Disclosure indicates that the app developer ignore disclosure of specific data items governed by Apple Privacy Label requirements. For example, xxx. 
%
To understand the pervasiveness of Omitted Disclosure, we utilize the formalization definition in XXX, let \source{} to be $s:(d_{s},p_{s})$ xxx.  \XY{need rewrite refer to section3}
%
Among xxx apps, we found xxx apps omitted to disclose xxx data objects (on average xxx data objects per app). Specially, xxx apps failed to disclose xxx data objects for the purpose (Third-party adverting, Developer’s Advertising or Marketing, Analytics).
%
The results indicate that most app developers are unable to deliver complete data disclosure in privacy label. 



\vspace{2pt}\noindent\textbf{analysis of omitted data types and purposes.}
To understand what kind of data under which purpose are prone to be ignored by app developer, we present the top 20 omitted data ranking by the number of apps under four purposes, as shown in \ref{fig:omit}. 
%
Under the purpose of Third-party Advertising, the device ID and location data are most prone to be omitted by the developer. Those data are commonly used by third-party advertising SDKs to track users and fine-tune the ads that show to a user. Unexceptionally, user profile information like email address, phone number, age, and gender are also ranked at the top, which can be used to profile users to perform targeted advertising.
%
For the Developer's Advertising or Marketing purpose, similar to before, advertising-related data (e.g., advertising identifier, location, etc.) are also prone to be neglected. Besides, the developers tend to send promotion and marketing campaigns to users and the text message (ranked top 3) responded through customer support services are also being collected for its own promotion purpose.
%
For the purpose of Analytics, the top one omitted disclosure data is demographic information, which can be used to understanding audience composition in terms of gender, age, and interests. Besides, analytic-specific data are also recklessly ignored to disclose (e.g., traffic information, log information, performance information etc), which can be used to evaluate user behavior, analyze product features or measure audience size. 
%lets you also understand the kinds of creative content you need to develop, the kinds of media buys you should make, and the kinds of audiences you need to develop for marketing and remarketing campaigns --\url{https://support.google.com/analytics/answer/2819950#zippy=%2Cin-this-article}
%
For app functionality, the identified omitted-disclosed data are commercially confidential (e.g., payment card information) or personal sensitive (e.g., ssn, employment information). 
%
The results show that the omitted data types are tightly correlated with its purpose, which also reflects the accuracy of our method. 






\subsubsection{Incorrect Disclosure}
Incorrect Disclosure indicate that the app developer try to declare this piece of data usage in privacy label, but struggle to correctly disclose the purpose. For example, xxx.  
%
To understand the pervasiveness of Incorrect Disclosure, we utilize the formalization definition in XXX, let \source{} to be $s:(d_{s},p_{s})$ xxx.   \XY{need rewrite refer to section3}
%
The result shows that 9791 apps incorrectly label the purposes of xxx data objects. 

\vspace{2pt}\noindent\textbf{analysis of incorrect Disclosure data types and purposes.}
As shown in figure XXX, the most prevalent incorrect disclosed purpose pair is xxx and xxx. The definition of xxx(purpose) is xxx, and the definition of xxx(purpose) is xxx. The boundary between xxx and xxx may be too ambiguous for developer to make correct decision. We also observe that xxx app developers tend to to distrustfully disclose purpose to be App functionality, while in fact it is used for advertising. Such incorrect disclosure betrays user's trust and may intentionally deceive user to download and use their app by claiming they have more acceptable reason to collect user data. As revealed in \cite{brush2010exploring}, user were very willing to share their location data to help cities plan bus routes or to get traffic information (\textbf{App functionality}), but reluctant to share the same data for ads (\textbf{Advertising}) or for maps showing one’s travel patterns (\textbf{Analytics}) \cite{bui2021consistency}. As to data types, we found the most likely to be incorrectly disclosure are XXX, which indicated that XXX. 



\subsubsection{Inadequate Disclosure}
Inadequate Disclosure means the developer has already declared one or multiple purpose for a specific data item, but failed to comprehensively disclose all of them. For example, xxxx. 
%
To understand the pervasiveness of Inadequate Disclosure, we utilize the formalization definition in XXX, let \source{} to be $s:(d_{s},p_{s})$ xxx. \XY{need rewrite refer to section3}
%
The result shows that xxx apps inadequately label the purposes of xxx data objects, which indicated that xxx.

\vspace{2pt}\noindent\textbf{analysis of Inadequate Disclosure data types and purposes}. As shown in figure XXX, the most 
prevailing inadequate purpose is XXX. Under this purpose, the most frequent data type is XXX. The results indicate that xxx. 


\subsection{Reasons of Inconsistency }

\vspace{2pt}\noindent\textbf{Data scope and granularity}. 
First, different data scope could cause some data in privacy policy are unable map to privacy label. As mentioned before, Apple defined a limited set of data items (32) for developers to disclose in privacy label. Differently, required by the law regulators (e.g., GDPR \cite{}, FTC \cite{} etc.), the app developer need to disclose all information relating to an identified or identifiable natural person in privacy policy. Consequently, some data items in privacy policy may not be able to find an appropriate data definition in privacy label. For example xxx. 
%
Second, different data granularity could cause some data is difficult to correctly map from privacy policy to privacy label. Apple required the developer to refer to pre-defined 32 data types and compare them to the data collection practices. Some data item are defined at specific way (e.g., email address) which is clearly for developer to identify; while some other data items defined at a broad semantic granularity (e.g., Sensitive Info) which required developer to know what kind of data is semantically subsumptive to it. %
In our study, XXX inconsistent cases are caused by this reason xxx. 


\vspace{2pt}\noindent\textbf{Privacy policy vagueness and generalization }
First, the vague expression of collection in privacy policy and the explicit collection in privacy label regarded to the same data could cause inconsistency. Specifically, in privacy policy, the ``collect'' action in some policy statement is modified by auxiliary verb (e.g., may, could, might) or adverb (e.g., possibly), which indicates that it is uncertain whether such data collection will happen or not. For example, xxx. 
%
Different from privacy policy, each data collection and usage in privacy policy is explicit and determined. 
%
Second, the privacy policy is general for all services/software provided by one company, while privacy label is tailored for a specific app. For example xxx. 
%
In our study, XXX inconsistent cases are caused by this reason xxx. 

\vspace{2pt}\noindent\textbf{Lack an understanding of privacy-best practices }
Mis-understanding the disclosure requirements in privacy label could cause inconsistency in privacy policy. Cranor’s research group pointed out that app developers had trouble creating accurate labels for their apps because they didn’t understand all the terminology and policy \cite{consumerreports}. 
%
Apple define an optional disclosure where certain data types that meet all of the following criteria are optional to disclosure (1. the data is not used for tracking purposes; 2. the data is not used for Third-Party Advertising; 3. infrequently collection; 4. user awareness). The developers may wrongly take for granted that meeting one of criteria can be optionally disclosed. 

%For example, data collected on an ongoing basis after an initial request for permission must be disclosed

Beside, Apple offer the option ``Data Not Collected'' label for app developer to fill if the app didn't collect any data. However, the app developer could just simply fill out this statement in privacy label for convenience. In our study, XXX inconsistency are caused by this reason xxx. 

\ignore{Cranor’s research group at Carnegie Mellon University conducted studies on Apple’s privacy labels with both app developers and consumers, and uncovered major shortcomings. “We found that, in general, people really like the idea of the labels but that there is a lot of confusion,” Cranor says. Developers in the studies had trouble creating accurate labels for their apps because they didn’t understand all the terminology, she says, while “the consumers didn’t know the labels existed until we pointed them out.” \url{https://www.consumerreports.org/privacy/google-adds-privacy-labels-to-apps-but-will-they-help-a3062366269/}
}


%many developers struggle to understand what type of data third par- ties receive, and with limited time and resources even self- described privacy advocates and security experts grapple with implementing privacy and security protection (Balebako et al. 2014)

%https://www.researchgate.net/publication/269197012_The_Privacy_and_Security_Behaviors_of_Smartphone_App_Developers
\subsection{Trend of Inconsistency }

With the evolution of the privacy label over time and Apple claimed that they devote themselves to providing resources for developers to help them fill out this information accurately~\cite{privacylabelsupport}. However, whether the privacy label becomes more accurate or more faulty is unclear. To investigate this problem, we perform a longitudinal study on XXX snapshots of privacy label and privacy policy. Specifically, given a snapshot of a set of privacy label, we first obtain its corresponding privacy policy by retrieving privacy policy link from each app's privacy label page. Further, we input privacy label and privacy policy into our \policycompaer{} module. The results are plot in the figure XXX. The x-axis is the timeline and y-axis is the number of apps existing inconsistency problems. The results showed that XXX

==> main/7.discussion.tex <==
\section{Discussion}

This is a sample! 
lessons

1. SDKs provide configuration options to disable tracking or advertising or analytics, but app developer usually ignore them. 

2. The privacy label guideline provided by the third-party SDKs are either incomplete, misleading or even incorrect, which caused the app developer are confusing how to declaim correct label

3. the guideline of apple privacy label is too coarse. 

4. different granularity of sensitive data in privacy label and those defined by GDPR?

\xiaojing{deal with the data items not covered by this paper}

\LXcomment{might discuss those data items that we did not cover.}




% (e.g., a misconception about Data Linked to Users)
%They pinpoint the challenges for developers to provide accurate privacy label and provide recommendations for the standardize privacy label .

==> table/cloudmall.tex <==

\begin{table}[ht]
\centering
\footnotesize
\caption{cloudmall network traffic}
\begin{tabular}{c|c|c}
\hline
\textbf{Company} & \textbf{Leaked data} & \textbf{Endpoint} \\ \hline

Facebook SDK & \makecell{device ID, user ID,\\ user event information etc} &  \textit{graph.facebook.com} \\ \hline

Adjust SDK & \makecell{IDFA, IDFV} &  \textit{app.adjust.com} \\ \hline

%Onesignal SDK & \makecell{geographical location, email,\\ advertising identifier,\\ user event information etc} &  \textit{api.onesignal.com} \\ \hline

Google SDK & \makecell{anonymous user id, email,\\ advertising IDFA, etc} &  \textit{app-measurement.com} \\ \hline


\end{tabular}
\label{table:cloudmall}
\end{table}

==> table/overviewExample.tex <==
\begin{table*}[ht]
\centering
 \vspace{15pt}
\footnotesize
\begin{tabular}{c|c|c|c|c}
\toprule
\textbf{Inconsistency Type} & \textbf{Endpoint} & \textbf{Data Collection (example)} & \textbf{Actual Purposes} & \textbf{Disclosed Purposes}\\ \hline

\multirow{2}{*}{Neglect Disclosure} & \makecell{https://www.google-analytics.com/\\collect?} & \makecell{ client\_id=8336016581650928698\\
ios\_jb=1, sz=300x250 \XY{to update}} & Analytics & -\\ \hline


\multirow{2}{*}{Contrary Disclosure} & \makecell{https://pubads.g.doubleclick.net\\/gampad/ads?} & \makecell{rdid=5B30BC06-9017-4FA0\\-8A77-3FB3FFBE3D7D} & Third-Party Advertising & App Functionality\\ \hline
 


\multirow{3}{*}{Inadequate Disclosure} & \makecell{https://aax-us-east.amazon\\-adsystem.com/e/msdk/ads?} & \textit{\makecell{``geoloc'':``39.154663, -86.492607, \\65.000000, 1''}} & Third-Party Advertising & \multirow{3}{*}{App Functionality} \\ \cline{2-4}
 & \makecell{https://api.tegnadigital.com/mobile/\\configuration-ro/updateUserLocation?} & \makecell{"lastKnownCoordinates":\\\{"latitude":39.136590224210444,\\"longitude":-86.48033368434717\}} & App Functionality & \\ \bottomrule
\end{tabular}

\caption{Three inconsistencies in app \textit{Atlanta News from 11Alive}}
\label{table:overviewExample}
\end{table*}

==> table/pattern.tex <==

\begin{table*}[ht]

\centering
\footnotesize
\caption{Summary}
\begin{tabular}{c|c|c|c|c|c|c|c|c|c}
\hline
Caller & API  & Frequency  & Endpoint Role$^\ddag$    & Request & Response  & First Level Property& Second Level Purpose &OP$^\dag$\\ \hline


App  & System API   &only once   & ADC& AUI $\wedge$ PII &  RED  & Data linked to the user &App functionality &Y  \\\hline

Third-party  & System API  & Frequently   & TAD  & FADI $\wedge$ PII & TAD   & Data linked to the user &Third-Party Advertising &N \\\hline

Third-party  & System API  & Frequently   & TAN & UBI $\wedge$ PII & MD  & Data linked to the user & Analytics &N \\\hline

App $\vee$ Third-party  & System API  & Frequently   & ADC $\vee$ TAM & TADI $\wedge$ PII & MM $\vee$ FAD  & Data linked to the user & Developer’s Advertising or Marketing &N \\\hline
 \\\hline
 
\end{tabular}
\begin{flushleft}
$\dag$: Optional Disclosure.\\
$\ddag$: Endpoint Role: Third-party Advertiser:TAD,  Third-party analytics: TAN, Third-party measurement or marketing: TAM, App Developer Company: ADC, Third-party app maker: TAM.
%Android 10 additionally requires a \texttt{XXX} permission when XXX in the backgroud.} \haoran{please fill and check.

\end{flushleft}
\label{table:pattern}
\end{table*}

==> table/privacyLabelBreakdown.tex <==
\begin{table}[t]
\centering
\footnotesize
\caption{Break down the privacy label into purpose of data usage and data item collection in ``Data Linked to you'' and ``Data used to Track you'' data category \xiaojing{update the number using $\mu\pm\sigma$}}
%\xiaojing{only focus on data linked to you and data used to track you}}
\begin{tabular}{c|c|c}
\hline
\hline

\textbf{Privacy Label Category} & \textbf{Item} &  \textbf{\# app ($\mu\pm\sigma$)} \\ \hline \hline

%\multirow{4}{*}{Categories of data usage} & Data Not Linked to You & 91,720 $\pm$ 5,023 \\ \cline{2-3}  & Data Linked to You  & 73,331 $\pm$ 5,053
%\\ \cline{2-3}   & Data Not Collected & 56170 $\pm$ 2,553
%\\ \cline{2-3} & Data Used to Track You & 48,631 $\pm$ 2,607 \\ \hline

\multirow{6}{*}{Purpose of data usage} & App Functionality & 61,937 $\pm$ 4,526 \\ \cline{2-3}  & Analytics  & 43,167 $\pm$ 3,048 \\ \cline{2-3}  & Product Personalization & 29,157 $\pm$ 2,061 \\ \cline{2-3} & \makecell{Developer’s Advertising \\ or Marketing} & 21,705 $\pm$ 1,540 \\ \cline{2-3} & Third-Party Advertising & 20,500 $\pm$ 970 \\ \cline{2-3}   & Other Purposes &  8,937 $\pm$ 671 \\\hline

\multirow{5}{*}{\makecell{Data types \\ (top 5)}} & Identifiers & 66,646 $\pm$ 4,392 \\ \cline{2-3} & Usage Data & 50,468 $\pm$ 3,316  \\ \cline{2-3}  &  Contact Info & 47,916 $\pm$ 3,728\\ \cline{2-3} & Diagnostics & 30,893 $\pm$ 2,132 \\ \cline{2-3}    & Location & 29,340  $\pm$ 1,933 \\\hline

\multirow{5}{*}{\makecell{Specific data items \\ (top 5)}} & Device ID &  50,454 $\pm$ 3,051 \\ \cline{2-3} &  User ID & 44,756 $\pm$ 3,290 \\ \cline{2-3} & Email Address & 40,635 $\pm$ 3,489 \\ \cline{2-3}  & Product Interaction &  38,406 $\pm$ 2,754  \\ \cline{2-3}    & Name &  36,986 $\pm$ 3,129 \\\hline


\end{tabular}
\label{table:labelBreakdown}
\end{table}


==> table/request.tex <==

\begin{table}[ht]
\centering
\footnotesize
\caption{Request}
\begin{tabular}{l|c}
\hline
authorization information (AUI) & access\_token,oauth\_service \\ \hline
personal information (PII) & email, first\_name,last\_name, address, city, postcode, country,gender   \\ \hline
advertising information (ADI) & adurl, adslots, is\_origin\_ad, publisher\_timeout\_control, idfv,  ad\_sdk\_version, accepted\_size, width, height, ad\_count,fbs\_aeid, skadn\_registered\_at\\ \hline
user behavior information (UBI) & log time, xwhen, xwho, xwhat, is\_first\_day, is\_login, first\_visit\_time, first\_visit\_language, is\_from\_background,subscription\_start\_date \\ \hline


\end{tabular}
\label{table:request}
\end{table}

==> table/response.tex <==

\begin{table}[ht]
\centering
\footnotesize
\caption{Response}
\begin{tabular}{l|c}
\hline
registration data (RED)  & create time \\ \hline
first party advertisement data (FAD) & xxx \\ \hline
measurement data (MD) & xxx \\ \hline
third party advertisement data (TAD) & xxx \\ \hline
marketing metrics (MM) & xxx \\ \hline

\end{tabular}
\label{table:request}
\end{table}

==> table/topAdvertiser.tex <==

\begin{table}[ht]
\centering
\setlength{\tabcolsep}{3.6pt}{% 调整列间距
\footnotesize
\caption{Top Advertsing, Analytics, Marketing parties}
\begin{tabular}{l|c|c|c}
\hline
\textbf{Company} & \textbf{Leaked data} & \textbf{Endpoint} & \textbf{\#}\\ \hline

\scriptsize\makecell{ Google\\ Analytics~\cite{firebase}} &  \makecell{\scriptsize User ID, Device ID \\ \scriptsize Email Address etc} &  \textit{\makecell{\scriptsize app-measurement\\\scriptsize google-analytics.com}} & 1,062\\ \hline


\scriptsize Facebook~\cite{facebookGraph} &  \makecell{\scriptsize Device ID, User ID,\\
\scriptsize Coarse Location\\
\scriptsize Other Diagnostic Data} &  \textit{\makecell{\scriptsize www.facebook.com\\ \scriptsize graph.facebook.com\\\scriptsize web.facebook.com}} &704 \\ \hline


\scriptsize Google Ads~\cite{googleAdvertising} &  \makecell{\scriptsize Device ID, User ID,\\
\scriptsize Advertising Data,\\
\scriptsize Other Diagnostic Data} &  \textit{\makecell{\scriptsize ad.doubleclick.net\\ \scriptsize pubads.g.doubleclick.net\\\scriptsize googleads.g.doubleclick.net}} & 415\\ \hline




\scriptsize Branch.io~\cite{branchio} &  \makecell{\scriptsize User ID, Device ID \\ \scriptsize Other Data Types etc} &  \textit{\makecell{\scriptsize api.branch.io \\ \scriptsize api2.branch.io}} &97 \\ \hline


\scriptsize Adjust~\cite{adjust} & \makecell{\scriptsize User ID, Device ID \\ \scriptsize Precise Location etc} &  \textit{\makecell{\scriptsize app.adjust.com\\\scriptsize view.adjust.com}}&66 \\ \hline

\end{tabular}
\label{table:topAdvertiser}}
\end{table}

==> table/topAppMaker.tex <==

\begin{table}[ht]
\centering
\setlength{\tabcolsep}{4.5pt}{% 调整列间距
\footnotesize
\caption{Top App Maker \xiaojing{remove}}
\begin{tabular}{l|c|c|c}
\hline
\textbf{Company} & \textbf{Leaked data} & \textbf{Endpoint} & \textbf{\#}\\ \hline



\scriptsize com.goodbarber &  \makecell{\scriptsize User ID,\\ \scriptsize Precise/Coarse Location,\\ \scriptsize Other Diagnostic Data,} &  \textit{\makecell{\scriptsize api.ww-api.com}} & 85\\ \hline

\scriptsize com.greencopper &  \makecell{\scriptsize Sensitive Info} &  \textit{\makecell{\scriptsize user-state.greencopper.com}}& 18\\ \hline

\scriptsize com.appypie &  \makecell{\scriptsize Device ID, User ID,\\\scriptsize Other Diagnostic Data,\\ \scriptsize Coarse Location} &  \textit{\makecell{\scriptsize api.appexecutable.com}} & 15\\ \hline

\scriptsize com.yinzcam  &  \makecell{\scriptsize Advertising Data} &  \textit{\makecell{\scriptsize ads-min-mls.yinzcam.com}}& 5\\ \hline




%\scriptsize com.makeitapp  &  \makecell{\scriptsize User ID,\\\scriptsize Precise/Coarse Location} &  \textit{\makecell{\scriptsize api.makeitapp.com}}& \\ \hline


\end{tabular}
\label{table:appMaker}}
\end{table}
